Views Can Be Deceiving: Improved SSL Through Feature Space Augmentation

Supervised learning methods have been found to exhibit inductive biases favoring simpler features. When such features are spuriously correlated with the label, this can result in suboptimal performance on minority subgroups. Despite the growing popularity of methods which learn from unlabeled data, the extent to which these representations rely on spurious features for prediction is unclear. In this work, we explore the impact of spurious features on Self-Supervised Learning (SSL) for visual representation learning. We first empirically show that commonly used augmentations in SSL can cause undesired invariances in the image space, and illustrate this with a simple example. We further show that classical approaches in combating spurious correlations, such as dataset re-sampling during SSL, do not consistently lead to invariant representations. Motivated by these findings, we propose LateTVG to remove spurious information from these representations during pre-training, by regularizing later layers of the encoder via pruning. We find that our method produces representations which outperform the baselines on several benchmarks, without the need for group or label information during SSL.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> methods.tex <==
\begin{figure*}[tpb]
\centering
\vspace{-1em}
\includegraphics[width=0.7\textwidth]{ssl/figure1.pdf}
\vspace{-.5em}
\caption{
% \textbf{
We use model transformation modules to create new views of training examples in the representation space. The introduced set of transformations removes the features learned in the final few layers, and provides final representations invariant to such transformations. 
% }. 
% Two augmented views of one image are processed by the same encoder network $f$ (a backbone plus a projection MLP). Then a prediction MLP $h$ is applied on one side, and a stop-gradient operation is applied on the other side. The model maximizes the similarity between both sides.
\label{fig:main}
\vspace{-.8em}
}
\end{figure*}

% \section{Methods} 
\section{\textbf{L}ate-layer \textbf{T}ransformation-based \text{V}iew \text{G}eneration }
\todo{mention we propose feature modification, or augmentations in the representation space, is a way of combating spurious connectivity in the augmentation graph in the representation space, remove the mathy part and add it to appendix instead}

%\subsection{Problem Setup} % TODO: summarize -- comment out everything else other than notation for image space, representation space, pretext and downstream tasks DEFINE all notation used in the next subsection


% If we assume that $z_\text{spur}$ is easier to learn, and majority examples can be discriminated by this feature as well as $z_\text{core}$, the core feature may not be fully captured in SSL representations. However, if the positive pairs have the same $z_\text{core}$ but different or removed $z_\text{spur}$, the encoder must learn the core features~\cite{robinson2021can}.

We found that spurious correlations in underlying latent features, can result in with usual augmentations used in visual self-supervised learning methods. Instead of curating specific image augmentations that corrects for these biases in the image space, we propose the following approach. 
motivated by improved SSL model invariance when trained with augmentations in \emph{image} space~\cite{chen2020simple}, we propose a model transformation module that specifically targets augmentations that modify the spurious feature in \emph{representation} space. We propose \textbf{L}ate-layer \textbf{T}ransformation-based \text{V}iew \text{G}eneration - \ours, which uses transformations to overcome spurious learning in SSL models and improve core feature representation.


% \subsection{
\emph{\textbf{L}ate-layer \textbf{T}ransformation-based \text{V}iew \text{G}eneration }
% -- Late-TVG
% }
\label{sec:method}
%In the previous section, we found that overparameterized encoders can fail when there are certain minority groups within the training samples, and that the final layers of the model tend to be more predictive of the spurious feature. 
Formally, we consider a model transformation module $\mathcal{U}$, that transforms any given function $f_\theta$
parameterized by $\theta = \{W_1, \dots, W_n\}$ 
to 
% $\tilde{f}_\theta$
${f}_\tilde{\theta}$. At each step, we draw a transformation $\phi_{M, \theta'}$ form $\mathcal{U}$ 
% where  ${f}_{\tilde{\theta}} = \phi_{M, \theta'}(f_\theta)$. 
to obtain transformed encoder ${f}_{\tilde{\theta}}$ from $f_\theta$. 
Each model transformation can be defined with a mask $M \in \{0, 1\}^{|\theta|} = \{M^1, \dots, M^n\}$, where we re-parameterize the unmasked weights $(1-M) \odot \theta'$ (either reinitialize or set them to 0), and keep the rest of the weights  $M \odot \theta$  the same, thus
$\tilde{\theta} = \phi_{M, \theta'}(\theta) =  M \odot \theta + (1-M) \odot \theta'$.

\textbf{Transformations:} In our experiments, we consider a Threshold pruning transformation module. Threshold Pruning (\textbf{SSL\textsubscript{Prune, L, a}}): Magnitude pruning $a\%$ of the weights in all layers deeper than $L$: 
    %  \vspace{0.1in}
     $\mathcal{U}_\text{\;Prune, L, a} = \{\phi_{M_{L, a}, \theta_0} ; \theta_0 = (0)^{|\theta|} \} $ where $M_{L, a} = \{M^l_L \odot \text{Top}_{a}(W_l) \mid  l \in [n]\}$ and 
    $\text{Top}_{a}(W_l)_{i, j} = \mathbb{I}(W_l_{(i, j)} \text{ in top } a\% \text{ of } \theta) $.
    
% of re-initializations, or the singleton of unstructured magnitude pruning of the final layers, defined as below:
% \vspace{-0.1in}
% \begin{itemize}
    % \item Re-initialization of the final-layers (\textbf{SSL\textsubscript{Reinit, L}}): Re-initializing the weights in layers deeper than $L$: 
    % $\mathcal{U}_\text{\;Reinit, L} = \{\phi_{M_L, \theta_{\text{Reinit}}} \mid \theta_\text{Reinit} \sim \mathcal{D}_\theta \}$ where $M_L$ is masking all weights before layer $L$ or $M_L = \{M^l_L \mid M^l_L = \mathbbm{1}(l < L)^ {|W_l|}, l \in [n]\}$, and $\mathcal{D}_\theta$ is the parameter initialization distribution.
     % \item
    %  Threshold Pruning is magnitude pruning $a\%$ of the weights in all layers deeper than $L$: 
    % %  \vspace{0.1in}
    %  $\mathcal{U}_\text{\;Prune, L, a} = \{\phi_{M_{L, a}, \theta_0} ; \theta_0 = (0)^{|\theta|} \} $ where $M_{L, a} = \{M^l_L \odot \text{Top}_{a}(W_l) \mid  l \in [n]\}$ and 
    % $\text{Top}_{a}(W_l)_{i, j} = \mathbb{I}(W_l_{(i, j)} \text{ in top } a\% \text{ of } \theta) $


% \end{itemize}
%  is $\mathcal{U}_\text{\;Reinit, L} = \{\phi_{M_L, \theta_{\text{Reinit}}} \mid \theta_\text{Reinit} \sim \mathcal{D}_\theta \}$ where $M_L$ is masking all weights before layer $L$ or $M_L = \{M^l_L \mid M^l_L = \boldsymbol{\mathbb{I}}(l \le L)^ {|W_l|}, l \in [n]\}$, and $\mathcal{D}_\theta$ is the parameter initialization distribution. 

% move to first paragraph
To learn these representations, given two random augmentations $t, t' \sim \mathcal{T}$ from the augmentation module $\mathcal{T}$, two views $x_1 = t(x)$ and $x_2 = t'(x)$ are generated from an input image $x$. At each step, given a feature encoder $f$, and an augmentation module $\mathcal{U}$, we obtain a transformed model $\tilde{f} = \phi(f), \; \phi \sim \mathcal{U}$. 
During training, one example $x_1$ and $x_2$ are respectively passed through the normal encoder $v_1 = f(x_1)$, and the transformed encoder $\tilde{v}_2 = \tilde{f}(x_2)$. Encoded feature $\tilde{v}_2$ is now a positive example that should be close to $v_1$ in the representation space 
% \newcommand{\lnorm}[1]{\frac{#1}{\left\lVert{#1}\right\rVert _2}}
(see Appendix~\ref*{app:exp_setup}).
% = - \lnorm{h(v_1)}{\cdot}\lnorm{\tilde{v}_2}$

% TODO: re-write, add citations
% Note that these transformation modules are designed to avoid memorization, by removing the undesired information in the final layers, so that the output of the transformed module to be close to the original encoded examples in the representation space. 
% In other words, the model should be invariant to model transformations in the feature space, and thus these transformations can be considered as curated view generating operations for the minority groups. 
Similarly to Image Augmentation modules inducing representation space invariance based on visual similarities, View Generation modules encourage the encoder to be invariant to final layer transformations. We hypothesize that this enables learning more complex features in the earlier layers of the encoder. 
% ~\cite{abnar2021exploring}. % As a result, minority examples are 


==> tables/encoders-in.tex <==
\begin{table}[]
\label{table:encoders-in}
\caption{Worst-group accuracy (\%) of models pre-trained on large datasets when evaluated on datasets containing spurious correlations with a linear probe.}
\resizebox{\linewidth}{!}{
\begin{tabular}{@{}crrrr@{}}
\toprule
             & \textbf{CLIP} & \textbf{ERM\textsubscript{in}} & \textbf{SimCLR\textsubscript{in}} & \textbf{SimSiam\textsubscript{in}} \\ \midrule
\ds{cmnist}     & \textbf{88.9}                                & 85.4                                  & 85.5                                     & 86.4                                      \\
\ds{metashift}  & \textbf{83.1}                                & \textbf{83.1}                                  & 79.7                                     & 69.5                                      \\
\ds{waterbirds} & 81.1                                & \textbf{84.3}                                  & 78.8                                     & 79.2                                      \\ \bottomrule
\end{tabular}
}
\centering
\end{table}



==> tables/pruning_res.tex <==
% \begin{table*}[h]
%  \resizebox{.99\textwidth}{!}{
% \begin{tabular}{@{}ccrrrrrrrr@{}}
% \toprule
% \multicolumn{1}{l}{}     & \multicolumn{1}{l}{} & \multicolumn{2}{c}{\textbf{kNN (Target)}} & \multicolumn{2}{c}{\textbf{LR (Target)}} & \multicolumn{1}{c}{\textbf{LR (Group)}} & \multicolumn{3}{c}{\textbf{Other Metrics}}     \\ \cmidrule(l){3-4} \cmidrule(l){5-6}  \cmidrule(l){7-7} \cmidrule(l){8-10}  
% \multicolumn{1}{c}{\textbf{Dataset}}  & \textbf{Method}     & \textbf{Worst Group}   & \textbf{Average}  & \textbf{Worst Group} &  \textbf{Average}  & \textbf{Average}      & \textbf{I(Z; Y)} & \textbf{I(Z; G)} & \textbf{L\textsubscript{align}} \\ \midrule
% \multirow{5}{*}{\texttt{cmnist}}      & SSL\textsubscript{Base}      
%        & \textbf{41.91\%}                                  & 86.72\%                                   & 37.61\%                                  & 83.67\%                                   & 85.92\%                                               & 8.56E-01                                   & 5.40E-05                                   & 1.148                                                \\
% % & 44.4\%       & 85.6\%   & 39.0\%       & 89.8\%          & 84.5\%        & 8.59E-01    & 8.82E-05    & 1.129    \\  
% & SSL\textsubscript{Reinit, 15}       & 33.90\%                         & 86.19\%                          & 42.37\%                         & 78.89\%                          & 79.72\%                                & 8.42E-01                          & 8.89E-01                          & 0.511                                    \\
%                                & SSL\textsubscript{Prune, 0.7, 19}  & 37.04\%                         & 88.49\%                          & \textbf{50.00\%}                         & 81.62\%                          & 82.07\%                                & 8.60E-01                          & 9.03E-01                          & 1.21                                    \\
%                                & SSL\textsubscript{Prune, 0.9, 18}  & 32.20\%                         & 89.04\%                          & 44.07\%                         & 84.32\%                          & 81.55\%                                & 8.54E-01                          & 9.02E-01                          & 1.12                                    \\
%                                & SSL\textsubscript{Prune, 0.99, 19} & 35.19\%                         & 88.31\%                          & 44.07\%                         & 79.64\%                          & 82.00\%                                & 8.51E-01                          & 8.73E-01                          & 0.947                                    \\
% \midrule
% \multirow{5}{*}{\texttt{metashift}}   & SSL\textsubscript{Base}      
%  & \textbf{28.82\%}                                  & 54.17\%                                   & \textbf{27.68\%}                                  & 66.57\%                                   & 65.00\%                                       & 1.07E-01                                   & 6.17E-02                                   & 0.848                                                \\
% % & 18.6\%       & 65.5\%   & 31.0\%       & 57.5\%          & 62.9\%        & 8.41E-02    & 8.43E-02    & 0.925    \\
%         & SSL\textsubscript{Reinit, 18}       & 21.38\%                         & 61.23\%                          & 18.64\%                         & 62.95\%                          & 66.52\%                                & 1.54E-03                          & 1.86E-01                          & 0.940                                  \\
%                                & SSL\textsubscript{Prune, 0.7, 17}  & 27.59\%                         & 60.09\%                          & 18.64\%                         & 63.09\%                          & 67.24\%                                & 1.31E-01                          & 1.89E-01                          & 0.958                                    \\
%                                & SSL\textsubscript{Prune, 0.8, 17} & 24.83\%                         & 58.66\%                          & 20.34\%                         & 64.95\%                          & 64.66\%                                & 7.37E-02                          & 1.58E-01                          & 0.955                                    \\
%                                & SSL\textsubscript{Prune, 0.9, 18}  & 25.52\%                         & 59.23\%                          & 18.64\%                         & 64.66\%                          & 65.52\%                                & 3.85E-02                          & 1.46E-01                          & 0.947                                    \\
% \midrule
% \multirow{5}{*}{\texttt{spurcifar10}} & SSL\textsubscript{Base}       
% & 22.12\%                                  & 57.05\%                                   & 36.24\%                                  & 60.36\%                                   & 52.02\%                                       & 1.96E+00                                   & 3.43E-03                                   & 1.072                                                \\
% % & 27.1\%       & 54.7\%   & 11.1\%       & 44.0\%          & 61.7\%        & 1.51E+00    & 4.68E-03    & 0.750    \\
% & SSL\textsubscript{Prune, 0.3, 18}  & 31.25\%                         & 61.60\%                          & \textbf{45.83\%}                         & 66.86\%                          & 48.91\%                                & 1.98E+00                          & 1.10E-05                          & 1.08                                   \\
%                                & SSL\textsubscript{Prune, 0.5, 18}  & 30.77\%                         & 58.44\%                          & 43.75\%                         & 66.23\%                          & 49.37\%                                & 2.06E+00                          & 1.98E-09                          & 1.05      \\
%                                & SSL\textsubscript{Prune, 0.7, 19}  & \textbf{35.42\%}                         & 58.06\%                          & 41.67\%                         & 65.80\%                          & 49.79\%                                & 2.03E+00                          & 2.30E-02                          & 1.04      \\
%                                & SSL\textsubscript{Prune, 0.9, 17}  & 25.00\%                         & 50.98\%                          & 39.58\%                         & 58.59\%                          & 48.66\%                                & 1.65E+00                          & 5.56E-05                          & 0.630                                    \\
%  \midrule
% \multirow{5}{*}{\texttt{waterbirds}}  & SSL\textsubscript{Base}       
% & \textbf{49.72\%}                                  & 53.40\%                                   & 48.04\%                                  & 56.18\%                                   & 87.45\%                                      & 8.63E-02                                   & 5.84E-01                                   & 0.867                                               \\
% % & 43.4\%       & 50.2\%   & 46.2\%       & 49.5\%          & 84.4\%        & 8.23E-03    & 5.41E-01    & 0.706    \\ 
% & SSL\textsubscript{Prune, 0.3, 17}  & 48.29\%                         & 50.59\%                          & \textbf{52.34\%}                         & 55.59\%                          & 86.54\%                                & 5.03E-02                          & 5.92E-01                          & 0.858                                    \\
%                                & SSL\textsubscript{Prune, 0.7, 17}  & 43.77\%                         & 54.99\%                          & 51.56\%                         & 62.10\%                          & 81.76\%                                & 7.86E-02                          & 5.72E-01                          & 0.873                                    \\
%                                &SSL\textsubscript{Prune, 0.8, 18}  & 35.83\%                         & 60.23\%                          & 50.78\%                         & 60.10\%                          & 84.10\%                                & 1.01E-01                          & 4.60E-01                          & 0.802                                    \\
%                                & SSL\textsubscript{Prune, 0.9, 17}  & 47.54\%                         & 50.88\%                          & 52.18\%                         & 57.82\%                          & 89.80\%                                & 9.63E-02                          & 0.595E-01                          & 0.702  \\ \bottomrule
% \end{tabular}
% }
% \caption{Top model transformations for each dataset; The learned representations in each case, we freeze the representations to evaluate the representations with: (i) average and worst-group of a 5-NN classifier (ii) Average and worst-group of a linear classifier (iii) Average accuracy of a linear classifier trained to infer the spurious feature (iv) Mutual information between representations and classes (v) Mutual information between representations and spurious feature (vi) Alignment loss~\cite{zhang2022correct} which is indicator of how close examples within the same class are in the representation space. In many cases, the worst-group accuracy of linear classifier is improved; in other cases kNN accuracy has improvements; } \label{tab:main}
% % change labels (core feature predictions) 
% % core feature prediction, core feature prediction, other information metrics [turn other metrics in the figure, make it decimal,  no accuracy 
% % extra column label that goes over accuracy at core feature prediction then skip a column then add accuracy label
% % make a graph of other metrics

% \end{table*}
% % \vspace{-0.2in}

==> tables/ssl-vs-sup.tex <==

\begin{table*}[h]
\centering
\caption{Accuracy (\%) of SSL models pre-trained on each dataset versus features of a supervised model.}
\begin{tabular}{@{}lrrrrrr@{}}
\toprule
              & \multicolumn{3}{c}{\textbf{Average}}                                                   & \multicolumn{3}{c}{\textbf{Worst-Group}}                                                             \\ \midrule
              & \textbf{SimCLR} & \textbf{SimSiam} & \textbf{Supervised} & \textbf{SimCLR} & \textbf{SimSiam} & \textbf{Supervised} \\ \cmidrule(l){2-4}  \cmidrule(l){5-7}  
\ds{celebA}       & 82.1                       & 81.9                        & \textbf{91.9}                        & 76.7                         & 77.5                          & \textbf{81.7}                                 \\
\ds{cmnist}       & 82.5                       & 82.1                        & \textbf{98.4}                        & 81.7                         & 80.7                          & \textbf{94.9}                                  \\
\ds{metashift}    & 55.1                       & 55.8                        & \textbf{89.8}                        & 45.5                         & 42.3                          & \textbf{83.5}                                  \\
\ds{spurcifar10} & 69.3                       & 75.1                        & \textbf{89.9}                        & 36.5                         & 43.4                          & \textbf{79.6}                                  \\
\ds{waterbirds}   & 47.5                       & 50.7                        & \textbf{67.9}                        & 43.8                         & \textbf{48.3}                          & 41.1                                  \\ \bottomrule
\end{tabular}
\end{table*}


